Semantic Specialisation of Distributional Word Vector Spaces using Monolingual and Cross-Lingual Constraints

We present Attract-Repel, an algorithm for improving the semantic quality of word vectors by injecting constraints extracted from lexical resources. Attract-Repel facilitates the use of constraints from mono- and cross-lingual resources, yielding semantically specialised cross-lingual vector spaces. Our evaluation shows that the method can make use of existing cross-lingual lexicons to construct high-quality vector spaces for a plethora of different languages, facilitating semantic transfer from high- to lower-resource ones. The effectiveness of our approach is demonstrated with state-of-the-art results on semantic similarity datasets in six languages. We next show that Attract-Repel-specialised vectors boost performance in the downstream task of dialogue state tracking (DST) across multiple languages. Finally, we show that cross-lingual vector spaces produced by our algorithm facilitate the training of multilingual DST models, which brings further performance improvements.

==> Notes.tex <==
\section{Progress Summary}

\begin{enumerate}

\item Set up Paragram experiment; prepared initial (distributional) word vectors for all four languages; PPDB constraint extraction procedures; SimLex-999 evaluation for all languages. 

\item Prepared all PPDB constraint set sizes for hyperparameter cross-validation. Created multilingual WS-353 similarity and relatedness splits used to produce Paragram validation scores. Hyperparameter optimisation ran for all languages, varying PPDB constraint set sizes and the Paragram regularization constant. The validation score is a good proxy for all languages apart from Russian (where it can't be used for choosing the best parameters). For this reason, we are always running Paragram for five epochs, as this suffices for convergence.    

\item Produced the cross-lingual correlation table which shows how well the produced rankings for each language correlate with the gold standard SimLex-999 rankings for other languages. 

\item Procured and set up BabelNet, which provides (aligned) word senses across many languages. Anders extracted mappings from our vocabularies to BabelNet word senses, as well as all sets of antonymous word senses. These were used to create sets of cross-lingual synonymy pairs for each language pair, as well as four monolingual and six cross-lingual sets of antonyms. 

\item Running Paragram over bilingual (or four-lingual) vector spaces with the BabelNet similarity constraints led to substantial improvements in semantic quality for non-English vector spaces. The most reasonable explanation is that pegging non-English word vectors to the high-quality English ones makes them substantially better. The cross-lingual correlation tables support this hypothesis, since the English vectors produce a better SimLex ranking for non-English languages than word vectors of those languages (even post semantic specialisation). 

\item The performance gains from counter-fitting persist in other languages. Monolingual and cross-lingual antonymy also improve the cross-lingual vector spaces. Due to large amounts of noise (in both PPDB and BabelNet), we perform counter-fitting using only antonyms, as including incorrect similarity constraints or enforcing vector space preservation preserves these artefacts.    

\end{enumerate}





\subsection{Recent Progress}

\begin{enumerate}

\item Implemented heuristics to remove orthographically equivalent words. Trained a slot-specific NBT-CNN with DSTC2+WOZ data using the strongest EN-DE-IT-RU vectors. Two major issues: a) need to translate the DSTC2 ontology to other languages; b) $n$-grams are very different across languages, i.e.~word order: \emph{adj noun} (EN) vs \emph{noun adj} (IT). Current model performance may indicate we are more likely to benefit from \emph{domain adaptation} rather than \emph{zero-shot transfer learning}. We also need to think about whether we translate ontologies and then apply the model to Italian dialogues and Italian target vectors (full transfer learning scenario), as opposed to inputting Italian dialogues, using Italian vectors but annotating with English labels (i.e.~using the original English ontology and English vectors as target labels). 

\item DONE: Ivan trained word vectors for DE, ES, FR, PT, NL, PL, SH, BG, SV. We extracted PPDB pairs and BN mappings for all of these (no PPDB for SH or SV). 

\item We pruned the sets of BabelNet constraints by ignoring BN senses which are named entities. This cut around 20\% of the constraints so it helped optimisation time. It also achieved marginal improvements in SimLex scores. 

\end{enumerate}







\subsection{Work in Progress}

\begin{enumerate}

% \item DONE: validation scores experiment - saving vectors which do the best: made sure this is a good strategy. Contacted John Wieting to ask for advice with hyperparameter tuning; got advice, regularization is very important, batch size is not (50-100). He does not seem to cross-validate to choose the best PPDB size. 

% \item DONE: validation score behaves well: it's a good proxy for SimLex-999 scores for German and Italian. The default XL and $10^{-9}$ seem to be the best choice, as suggested by John Wieting. Not the case for Russian: validation score exhibits anti-correlation with SimLex and PPDB-M works much better than PPDB-XL. 

% \item DONE: fixed mistake in normalisation which lowered English and Russian scores, and also made the WS-353 validation experiments for these languages a (much) worse estimator. Still not as good as German and Italian, though. 

% \item DONE: constraint sets which list cross-lingual word pairs belonging to the same BabelNet word senses. Ready for each language pair. 

% \item DONE: created merged sets of vocabularies and word vectors for each language pair (using the Paragram-ed word vectors as starting point).  

% \item DONE: ran Paragram with cross-lingual word pairs (EN-DE, EN-IT, DE-IT). In all cases, this lead to major SimLex improvements: especially for the 'lower resource' languages (IT, DE). Tuning using the average of the WS-353 validation scores of both languages. EN-IT uploaded to Dropbox: while these vector collections are not final (need antonyms before counter-fitting), we can run some preliminary experiments to gauge their usefulness for lexical entailment. 

% \item DONE: cleaned the four collections of word vectors further to remove all special characters, non-words and to standardise Unicode representations. 

% \item DONE: decided not to merge representations of orthographically equivalent words across languages. If we keep these separate, the initial SimLex scores stay the same as those in Table 1 (either pre/post Paragram), and it will be easier to understand what effect the injected cross-lingual constraints have.  

% \item DONE: included SimVerb list as potential validation or evaluation metric. Since its monolingual, maybe just evaluation. 

% \item DONE: start from monolingual distributional vectors and run Paragram over these using the two languages' monolingual paraphrases together with the cross-lingual BabelNet constraints. This would help with languages where monolingual validation was problematic (i.e.~Russian). Worked well for EN-IT: 0.57 for both languages (we get 0.59 for both when we start from Paragramed monolingual vectors).   

% \item DONE: removed Paragram validation criterion. Looking at word vectors update magnitude between epochs: when this stabilises, we deem the procedure has converged. Five epochs is typically sufficient for the update to converge. Planning to rerun monolingual experiment and generate Tables 1-3 from these vectors (vocabularies have also been modified).

% \item DONE: a lot of vocabulary pruning using OpenSubtitles. The large overlap (i.e.~\emph{north} in the Italian vocabulary) is problematic for DST experiments. Pruned all four vocabularies (preserving SimLex coverage of the original vectors). This speeds up the Paragram experiments (fewer vectors means fewer constraints to inject, dropping from 2.0M to 1.4M constraints). 

% \item DONE: Anders produced a list of antonymous BabelNet synsets. Used these, together with the previous lists, to produce antonym sets for each language pair. We have both monolingual and cross-lingual antonyms. In total, there are 53k antonyms in all of these sets.  

% \item DONE: merged all four word vector collections (distributional/Paragram). Prepared all constraints (with prefixes) for the universal word vectors: six sets of cross-lingual ones and four sets of monolingual ones. Starting from four sets of distributional word vectors and injecting 1.4 million constraints. Final EN-DE-IT-RU SimLex scores are [0.63, 0.57, 0.59, 0.54]. Counter-fitting with cross-lingual and multilingual antonyms (53k) raises these figures to [0.67, 0.59, 0.63, 0.55]. These two word vector collections have been uploaded to \url{mi.eng.cam.ac.uk/~nm480/final-vectors.txt.zip} and \url{../final-cf-vectors.txt.zip} The SimLex scores of these two collections on the original English SimLex are 0.69 and 0.71, respectively. Interestingly, counter-fitting with just antonyms (all of them) leads to [0.70, 0.61, 0.67, 0.55]. If we drop the VSP term, we get [0.70, 0.61, 0.67, 0.55], but the neighbourhoods look better (esp. difficult ones such as area). The 0.70 on new English SimLex corresponds to 0.74 on the old one. 

% \item DONE: go further than bilingual. All languages except English benefit from being linked to other languages. It would be interesting to see what happens when we mix all of the languages together. To do this, we need to merge all four sets of vectors, as well as all sets of monolingual and cross-lingual constraints. I also need to update the Paragram code (for validation across the four languages). 

% \item DONE: with the new vocabularies, I've rerun mono-Paragram and CF for Tables 1 and 2. German has become slightly due to smaller vocabulary.  

% \item DONE: Refactored the Neural Belief Tracker code. This model will be used for the dialogue state tracking experiments \cite{Mrksic:16b}. Adapted to Unicode and all the language prefixes.

% \item IN PROGRESS: translating dialogue ontologies. This doesn't help with (subjective) DST performance: labelling using the English ontology gives better performance. We can probably conclude that we need some in-domain data to "adapt" to the new ontologies. This will be clear once we collect some non-English data and perform tracking over it (as labels have a direct 1-1 mapping between languages). Italian ontology done, German and Russian left to do. 

% \item TODO: cross-lingual constraints on top of monolingual Paragram vectors. This should tell us more about cross-lingual gains (and it also had better performance for EN-IT).  

% \item TODO: could the huge cross-lingual effect be due to just word senses from BabelNet linking back to monolingual similarity? What happens if we inject just monolingual similarity constraints extracted from BabelNet (we haven't used these constraints any experiment so far). 

% \item DONE: Joint Synonym and Antonym injection (through the Paragram procedure). Code modified. PG + CF performance is attained (-0.01 for EN, IT, DE and RU all boosted by 0.01-0.02).  

\item IN PROGRESS: semantic specialisation by language group. We have one SimLex score as metric for Romance and Slavic, and two for Germanic (English and German). Germanic done, Romance and Slavic expected by 23 September. 

\item TODO: some sort of post-processing method to increase coverage in all of these languages? For example PG-A a large subset of (most common) distributional words, and then adapt the remaining, more sparse words to deal with things such as morphology. 


\item DONE: DST quick and dirty hack - we can translate the existing WOZ data into another language via Bing Translate. If we train with cross-lingual vectors, we can just apply the model to the translated DST dataset and check if the appropriate English labels are generated. Then, we can compare figures to the English ones, which are probably not perfectly attainable due to loss of meaning when utterances are translated, though I suspect this loss would not be very large. How much we lose in attempting the transfer is a more interesting question. Left to run for all twelve languages after WOZ is clean.

\end{enumerate}






\subsection{Joint Paragram + CF}

The Paragram algorithm minimises the following objective function. If $S$ is the set of synonymous word pairs, such that each word pair $(x_1, x_2) \in S$ corresponds to vectors $\mathbf{x_1, x_2}$, the cost function (sans normalisation and the regularization terms) is: 

\begin{align*}
\sum_{(x_1, x_2) \in S}  max\left(0, \delta_{sim} +  \mathbf{x_1} \mathbf{t_1} - \mathbf{x_1} \mathbf{x_2} \right) \\ 
                         max\left(0, \delta_{sim} +  \mathbf{x_2} \mathbf{t_2} - \mathbf{x_1} \mathbf{x_2}  \right)  
\end{align*}
The $\delta_{sim}$ hyperparameter is set to $0.6$, which means word vectors should be that much closer to their synonymous words' vectors than to the most similar of the 98 'randomly drawn' word vectors.

Here, the $\mathbf{t_1, t_2}$ terms correspond to word vectors of the \emph{negative examples} selected for the current paraphrase pair. Each mini-batch consists of 50 (configurable) paraphrase pairs, so for each word pair $\mathbf{(x_1, x_2)}$, two words are chosen to act as negative examples: $\mathbf{t_1}$ and $\mathbf{t_2}$, respectively. These words are chosen from the 100 words present in the current mini-batch. For each word, its negative example is the word with the \emph{most similar} word vector (apart from the other word in its paraphrase pair).    

To include antonyms (assume we have a collection of antonym pairs $A$), we propose adding analogous terms into the cost function:
\begin{align*}
\sum_{(x_1, x_2) \in A}  max\left(0, \delta_{ant} + \mathbf{x_1} \mathbf{x_2}  - \mathbf{x_1} \mathbf{t_1} \right) \\ 
                         max\left(0, \delta_{ant} + \mathbf{x_1} \mathbf{x_2}  - \mathbf{x_2} \mathbf{t_2} \right)  
\end{align*}
Here, for each word vector $\mathbf{x_1}$, we want the \emph{most different} word vector $\mathbf{t_1}$ of the 98 'randomly drawn' ones to be more similar to $\mathbf{x_1}$ than its antonymous vector $\mathbf{x_2}$, by a margin of at least  $\delta_{ant}$. So if the most different vector has a dot product of e.g.~$-0.4$, the distance between antonymous words would have to be at least $-0.4 - \delta_{ant}$. It may be sufficient to set this coefficient to $0.0$: with this hyperparameter, PG-A matches PG + CF. If we want to optimise performance, we could tune on SimVerb-3500 for English, and just use the same hyperparameters for other languages.   

\iffalse

\begin{enumerate}

\item German: downloaded and processed Wiki dump. \url{mi.eng.cam.ac.uk/~nm480/wiki.de.txt.tar.gz} 

\item French: downloaded and processed Wiki dump. \url{mi.eng.cam.ac.uk/~nm480/wiki.fr.txt.tar.gz} 
\item Serbian + Croatian: SR + HR + SH + BS combined and processed.  \url{mi.eng.cam.ac.uk/~nm480/wiki.yu.txt.tar.gz} 
\item Spanish: downloaded and processed Wiki dump. \url{mi.eng.cam.ac.uk/~nm480/wiki.es.txt.tar.gz} 
\item Dutch: downloaded and processed Wiki dump. \url{mi.eng.cam.ac.uk/~nm480/wiki.nl.txt.tar.gz} 

\item Portuguese: downloaded and processed Wiki dump.  \url{mi.eng.cam.ac.uk/~nm480/wiki.pt.txt.tar.gz} 
\item Polish: Downloaded and processed Wiki dump. \url{mi.eng.cam.ac.uk/~nm480/wiki.pl.txt.tar.gz} 

\end{enumerate}

\fi



\subsection{Future Work/Ideas/Considerations}

\begin{enumerate}


\item \textbf{Low resource languages}: improving SimLex scores of low resource languages by tying them to languages with more resources (i.e.~better distributional vectors, more/better similarity or antonymy constraints, etc.) The experiment could be English + German, where we do not use PPDB (or anything else) for German: we start from raw distributional vectors which we tie to the far more semantically specialised English ones. This is a great experiment since we do have the ceiling performance for German, i.e.~the German SimLex figures we get when we do use all the German resources to semantically specialise the word vectors.

\item \textbf{Other languages}: this one follows the low resource language experiment. We can get BabelNet and PPDB for other languages and run Paragram and counter-fitting to obtain semantically specialised vectors for those languages (e.g.~Spanish, French, etc.). We have eliminated the need for WS or SimLex for performing semantic specialisation. While we couldn't measure the semantic quality of vectors for these languages via SimLex, the cross-lingual experiments could be a good proxy. For example, if the Italian scores are improving when tied to French and Spanish, it is very likely that the word vectors for those languages will improve as well. Releasing semantically specialised word vectors for e.g.~10 languages could be a useful contribution in its own right. 
%On top of that, we could try to do DST for French using these vectors. 

\item \textbf{PG+CF - joint learning method}: especially in case of TACL, it would be good to show at least a modelling twist, since the current pipeline setup is clearly less than ideal. Performing synonymy and antonymy injection jointly while preserving strong performance would be ideal. We could try to redefine the skip-gram objective to incorporate the two types of constraints into the distributional model training. Similarity can be done via something similar to the Paragram objective, while antonymy could be done by always including antonyms as negative samples (i.e. \emph{improving} negative sampling). 

\item \textbf{DST data collection}: we need to collect annotated dialogues in another language (Shawn's Wizard of Oz experiment setup with Prolific Academic for German or Italian) and evaluate the dialogue state tracking performance. 

\item \textbf{Linguistic Depth / Analysis:} one of Roi's suggestions was to (for example) use a BabelNet cross-lingual constraint if and only if the words of the word pair share more than half of their word senses. Considerations such as these could give the paper more linguistic depth.

\item \textbf{Ivan's BLE experiment}: once we have word vectors we are happy with (perhaps the counter-fitted four-lingual ones), we should run Ivan's experiments again and find a good way to present those results.   

\item \textbf{SimLex score discrepancy:} why are SimLex scores lower for the new multilingual dataset? Fewer or different annotators? Empirically, the higher the scores are, the smaller the difference.


\end{enumerate}

% \item \textbf{Direct Downstream Applications:} text classification, parsing, sentiment analysis? Basically any application where we can use cross-lingual constraints to produce universal word vectors. We would use these vectors to train the task-specific model as in the monolingual scenario (i.e.~for a single high-resource language). We then evaluate the performance of this model for other (low-resource) languages. 

% \item \textbf{Multimodal learning}: learning representations across languages jointly? Does this make any sense due to different synsets/word senses across languages? 

% \item \textbf{Joint model training across domains:} also multimodal - we could perform a single task (i.e.~text classification, parsing, etc.) across different languages, training a model which just flips which word vectors it uses, but ties the model parameters. We could try also tuning or keeping word vectors fixed during this training procedure. 



\section{Results}

Distributional word vectors used as the starting point for each of the four languages:

\begin{enumerate}

\item \textbf{English}: using the largest GloVe Common Crawl vectors \cite{Pennington:14}. 

\item \textbf{German}: using Ivan's ACL vectors (trained on Polyglot Wiki?). Relatively weak performance (0.28). Will retrain word2vec model using German Wiki. 

\item \textbf{Italian}: we are using the CBOW vectors from \cite{Dinu:15}?

\item \textbf{Russian}: vectors downloaded from \url{ling.go.mail.ru/dsm/en/about}; we are using the smaller ones (300D). Larger ones have the same SimLex coverage (984 / 999) and a slightly better SimLex score.

\end{enumerate}

Table \ref{tab:cross-lingual-improvements} (first four sections) shows the effect of injecting monolingual semantic similarity constraints (from PPDB) via the Paragram procedure. It also shows the effect of then injecting monolingual antonymy constraints (extracted from BabelNet) via counter-fitting. It also shows the performance of the PG-A procedure, which incorporates antonymy injection into the Paragram procedure.  

Table \ref{tab:cross-lingual-improvements} shows the effect of injecting cross-lingual word sense similarity constraints from BabelNet in addition to the monolingual similarity constraints from PPDB. This semantic similarity specialisation step is done jointly; we will also do it sequentially (Paragram-ing PPDB constraints, evaluating, then injecting BabelNet constraints; and vice-versa) to better understand the effect of injecting cross-lingual word sense similarity (and find the best way to do it).


\iffalse

\begin{table} [!t]
\centering
\resizebox{1.0\columnwidth}{!}{%
\begin{tabular}{|c|c|ccc|}

\hline
Language & Coverage & Baseline & Paragram & + CF  \\
\hline
English & 998 & 0.32 & 0.55 & 0.63  \\
German & 934 & 0.28 & 0.39 & 0.42  \\
Italian & 984 & 0.36 & 0.46 & 0.54 \\
Russian & 984 & 0.38 &  0.54 & 0.57  \\
\hline
\end{tabular}%
}
\caption{SimLex-999 scores and the effect of mono-lingual similarity and antonymy injection.  \label{tab:simlex}} 
\end{table}


\fi



\subsection{Cross-lingual Correlation}

\begin{table} [hb]
\centering
\resizebox{1.0\columnwidth}{!}{%
\begin{tabular}{c|cccc}
~ & \bf English & \bf German & \bf Italian & \bf Russian \\  \hline
\bf English & 0.32 & 0.39 & 0.34 & 0.29  \\
\bf German & 0.22 & 0.28 & 0.21 & 0.20  \\
\bf Italian & 0.27 & 0.36 & 0.36 & 0.25  \\
\bf Russian & 0.32 & 0.35 & 0.36 & 0.38  \\
\end{tabular}%
}
\caption{the correlation of SimLex rankings induced from the distributional word vectors with the gold standard SimLex rankings of all four languages. Each row shows the correlation of the word vector subset representing the given language with the gold standard rankings of the four languages (columns). \label{tab:cross-lingual-correlation-original}} 
\end{table}





\begin{table} [hb]
\centering
\resizebox{1.0\columnwidth}{!}{%
\begin{tabular}{c|cccc}
~ & \bf English & \bf German & \bf Italian & \bf Russian \\  \hline
\bf English & 0.70 & 0.64 & 0.69 & 0.65  \\
\bf German & 0.63 & 0.62 & 0.62 & 0.58  \\
\bf Italian & 0.65 & 0.58 & 0.68 & 0.61  \\
\bf Russian & 0.60 & 0.54 & 0.58 & 0.61  \\
\end{tabular}%
}
\caption{the correlation of SimLex rankings induced from {the EN-DE-IT-RU cross-lingual word vectors} with the gold standard SimLex rankings of all four languages. Each row shows the correlation of the word vector subset representing the given language with the gold standard rankings of the four languages (columns). \label{tab:cross-lingual-correlation-original}} 
\end{table}



\iffalse

\begin{table*}
\def\arraystretch{1.0}
\centering
\small{
\resizebox{2\columnwidth}{!}{%
\begin{tabular}{c|c|cccccccccccc}
    & $|\mathtt{Vocab}|$& EN & DE & NL & SV & FR & ES & IT & PT & RU & PL & SH & BG \\ \hline
 EN & 76.8  & 640.4 & 246.3 & 305.5 & 207.8 & 358.0 & 317.4 & 356.5 & 255.4 & 196.3 & 275.6 & 186.7 & 136.0\\
 DE & 157.2  & 246.3 & 135.9 & 290.7 & 217.8 & 285.0 & 266.2 & 277.6 & 219.3 & 175.5 & 232.9 & 167.1 & 129.8\\
 NL & 158.5  & 305.5 & 290.7 & 681.4 & 241.9 & 347.8 & 316.5 & 340.8 & 258.3 & 199.7 & 278.7 & 200.2 & 146.9\\
 SV & 137.7  & 207.8 & 217.8 & 241.9 & 0.0 & 236.4 & 223.2 & 228.6 & 189.4 & 141.2 & 200.7 & 146.3 & 114.5\\
 FR & 199.6  & 358.0 & 285.0 & 347.8 & 236.4 & 1025.9 & 359.2 & 385.9 & 282.8 & 222.2 & 309.5 & 210.0 & 149.3\\
 ES & 164.4  & 317.4 & 266.2 & 316.5 & 223.2 & 359.2 & 1138.7 & 343.6 & 263.6 & 199.7 & 276.6 & 194.7 & 140.1\\
 IT & 178.9  & 356.5 & 277.6 & 340.8 & 228.6 & 385.9 & 343.6 & 159.3 & 277.5 & 221.0 & 297.3 & 208.1 & 149.1\\
 PT & 103.1  & 255.4 & 219.3 & 258.3 & 189.4 & 282.8 & 263.6 & 277.5 & 719.8 & 160.0 & 230.5 & 165.7 & 122.0\\
 RU & 252.9  & 196.3 & 175.5 & 199.7 & 141.2 & 222.2 & 199.7 & 221.0 & 160.0 & 48.6 & 169.4 & 115.8 & 88.4\\
 PL & 218.1  & 275.6 & 232.9 & 278.7 & 200.7 & 309.5 & 276.6 & 297.3 & 230.5 & 169.4 & 394.7 & 185.7 & 133.1\\
 SH & 168.7  & 186.7 & 167.1 & 200.2 & 146.3 & 210.0 & 194.7 & 208.1 & 165.7 & 115.8 & 185.7 & 0.0 & 99.2\\
 BG & 66.1  & 136.0 & 129.8 & 146.9 & 114.5 & 149.3 & 140.1 & 149.1 & 122.0 & 88.4 & 133.1 & 99.2 & 176.3\\
\end{tabular}}%}%
}
\caption{Synonymous constraint count (in thousands). For each language pair, the figure shows the number of synonymy constraints injected by the \textsc{Attract-Repel} procedure. Monolingual similarity constraints were extracted from PPDB, and cross-lingual similarity constraints were extracted from BabelNet. } \label{tab:constraint-count-syn}
\end{table*}

\begin{table*}
\def\arraystretch{1.0}
\centering
\small{
\resizebox{2\columnwidth}{!}{%
\begin{tabular}{c|c|cccccccccccc}
    & $|\mathtt{Vocab}|$& EN & DE & NL & SV & FR & ES & IT & PT & RU & PL & SH & BG \\ \hline
 EN & 76.8  & 5.5 & 11.2 & 16.7 & 10.7 & 20.1 & 17.3 & 24.3 & 14.1 & 9.2 & 14.6 & 12.4 & 7.2\\
 DE & 157.2  & 11.2 & 2.0 & 10.5 & 7.4 & 11.9 & 10.7 & 13.6 & 9.0 & 6.1 & 9.3 & 7.7 & 4.8\\
 NL & 158.5  & 16.7 & 10.5 & 4.0 & 10.4 & 16.9 & 15.3 & 19.8 & 12.9 & 8.3 & 13.1 & 11.8 & 6.6\\
 SV & 137.7  & 10.7 & 7.4 & 10.4 & 2.1 & 10.9 & 9.8 & 12.7 & 8.5 & 5.5 & 9.0 & 7.3 & 4.9\\
 FR & 199.6  & 20.1 & 11.9 & 16.9 & 10.9 & 5.3 & 17.8 & 24.5 & 14.5 & 9.5 & 15.0 & 12.8 & 7.3\\
 ES & 164.4  & 17.3 & 10.7 & 15.3 & 9.8 & 17.8 & 4.1 & 21.4 & 12.9 & 8.3 & 13.1 & 11.3 & 6.7\\
 IT & 178.9  & 24.3 & 13.6 & 19.8 & 12.7 & 24.5 & 21.4 & 7.9 & 17.7 & 11.1 & 18.0 & 14.9 & 8.8\\
 PT & 103.1  & 14.1 & 9.0 & 12.9 & 8.5 & 14.5 & 12.9 & 17.7 & 2.7 & 7.0 & 11.6 & 9.5 & 5.7\\
 RU & 252.9  & 9.2 & 6.1 & 8.3 & 5.5 & 9.5 & 8.3 & 11.1 & 7.0 & 1.3 & 7.1 & 6.1 & 3.6\\
 PL & 218.1  & 14.6 & 9.3 & 13.1 & 9.0 & 15.0 & 13.1 & 18.0 & 11.6 & 7.1 & 3.5 & 10.4 & 6.3\\
 SH & 168.7  & 12.4 & 7.7 & 11.8 & 7.3 & 12.8 & 11.3 & 14.9 & 9.5 & 6.1 & 10.4 & 3.3 & 5.0\\
 BG & 66.1  & 7.2 & 4.8 & 6.6 & 4.9 & 7.3 & 6.7 & 8.8 & 5.7 & 3.6 & 6.3 & 5.0 & 0.9\\
\end{tabular}}%
}
\caption{Antonymous constraint count (in thousands). For each language pair, the figure shows the number of antonymy constraints injected by the \textsc{Attract-Repel} procedure. Both the monolingual and cross-lingual antonymous constraints were extracted from BabelNet. } \label{tab:constraint-count-ant}
\end{table*}

\fi



\begin{table*}
\def\arraystretch{1.0}
\centering
\resizebox{2.07\columnwidth}{!}{%
{\small
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c}
& EN & DE & NL & SV & FR & ES & IT & PT & RU & PL & SH & BG \\ \hline

 EN  & 640,~~5 & 246,~11 & 305,~16 & 207,~10 & 358,~20 & 317,~17 & 356,~24 & 255,~14 & 196,~~9 & 275,~14 & 186,~12 & 136,~7\\
 DE  & 246,~11 & 135,~~2 & 290,~10 & 217,~~7 & 284,~11 & 266,~10 & 277,~13 & 219,~~8 & 175,~~6 & 232,~~9 & 167,~~7 & 129,~4\\
 NL  & 305,~16 & 290,~10 & 681,~~3 & 241,~10 & 347,~16 & 316,~15 & 340,~19 & 258,~12 & 199,~~8 & 278,~13 & 200,~11 & 146,~6\\
 SV  & 207,~10 & 217,~~7 & 241,~10 & ~~0,~~2 & 236,~10 & 223,~~9 & 228,~12 & 189,~~8 & 141,~~5 & 200,~~9 & 146,~~7 & 114,~4\\
 FR  & 358,~20 & 284,~11 & 347,~16 & 236,~10 & 1025,~5 & 359,~17 & 385,~24 & 282,~14 & 222,~~9 & 309,~14 & 210,~12 & 149,~7\\
 ES  & 317,~17 & 266,~10 & 316,~15 & 223,~~9 & 359,~17 & 1138,~4 & 343,~21 & 263,~12 & 199,~~8 & 276,~13 & 194,~11 & 140,~6\\
 IT  & 356,~24 & 277,~13 & 340,~19 & 228,~12 & 385,~24 & 343,~21 & 159,~~7 & 277,~17 & 220,~11 & 297,~18 & 208,~14 & 149,~8\\
 PT  & 255,~14 & 219,~~8 & 258,~12 & 189,~~8 & 282,~14 & 263,~12 & 277,~17 & 719,~~2 & 159,~~6 & 230,~11 & 165,~~9 & 121,~5\\
 RU  & 196,~~9 & 175,~~6 & 199,~~8 & 141,~~5 & 222,~~9 & 199,~~8 & 220,~11 & 159,~~6 & ~48,~~1 & 169,~~7 & 115,~~6 & ~88,~3\\
 PL  & 275,~14 & 232,~~9 & 278,~13 & 200,~~9 & 309,~14 & 276,~13 & 297,~18 & 230,~11 & 169,~~7 & 394,~~3 & 185,~10 & 133,~6\\
 SH  & 186,~12 & 167,~~7 & 200,~11 & 146,~~7 & 210,~12 & 194,~11 & 208,~14 & 165,~~9 & 115,~~6 & 185,~10 & ~~0,~~3 & ~99,~5\\
 BG  & 136,~~7 & 129,~~4 & 146,~~6 & 114,~~4 & 149,~~7 & 140,~~6 & 149,~~8 & 121,~~5 & ~88,~~3 & 133,~~6 & ~99,~~5 & 176,~0\\
 \end{tabular}}%
}
\caption{Linguistic constraint counts (in thousands). For each language pair, the two figures show the number of synonymy and antonymy constraints. Monolingual similarity constraints were extracted from PPDB, whereas cross-lingual similarity and both monolingual and cross-lingual antonymy were extracted from BabelNet. }

\label{tab:constraint-count}
\end{table*}




\begin{table}
%\def\arraystretch{1.0}
\centering
\small{
\begin{tabular}{c|cccc}
\bf Word Vectors & \bf EN & \bf DE & \bf IT & \bf RU \\ \hline
%\bf Monolingual Distributional Vectors & 0.32 & 0.28 & 0.36 & 0.38 \\ %\hdashline
%\bf Monolingual Constraints & 0.65 & 0.43 & 0.56 & 0.57 \\ \hline
%\bf EN, DE, IT, RU & 0.70 & \bf 0.62 & 0.68 & \bf 0.61 \\ \hdashline

%\bf EN & 0.65 &  - & - & - \\ \hline
%\bf DE-distributional & - &  0.28 & - & - \\ \hdashline
\bf DE-monoling-spec & - &  0.43 & - & - \\ \hdashline
\bf DE, NL & - & 0.55  & - & - \\ 
\bf DE, SV & - & 0.55 & - & - \\ 
\bf DE, NL, SV & - & 0.56 & - & - \\ \hdashline
\bf EN, DE, NL, SV & 0.70 & 0.61 & - & - \\ \hline 

%\bf IT-distributional & - & - & 0.36 & - \\ \hdashline
\bf IT-monoling-spec & - & - & 0.56 & - \\ \hdashline
\bf IT, FR & - & - & 0.68 & - \\ 
\bf IT, ES & - & - & 0.68 & - \\ 
\bf IT, PT & - & - & 0.66 & - \\ 
\bf IT, FR, ES, PT & - & - & \bf 0.69 & - \\ \hdashline
\bf EN, IT, FR, ES, PT & \bf 0.72 & - & \bf 0.69 & - \\ \hline 

%\bf RU-distributional  & - & - & - & 0.38 \\ \hdashline
\bf RU-monoling-spec & - & - & - & 0.56 \\ \hdashline
\bf RU, PL  & - & - & - & 0.60 \\
\bf RU, SH  & - & - & - & 0.59 \\
\bf RU, BG  & - & - & - & 0.61 \\
\bf RU, PL, SH, BG  & - & - & - & 0.59 \\ \hdashline
\bf EN, RU, PL, SH, BG  & 0.71 & - & - & \bf 0.61 \\ 

\end{tabular}}\caption{Multilingual SimLex-999. The effect of using the \textsc{Attract-Repel} procedure to inject monolingual or monolingual \emph{and} cross-lingual semantic constraints into combined collections of distributional vectors for various languages. } %In this table, we show that incorporating non-SimLex languages still leads to substantial gains over the monolingual scenarios, substantiating our intuition that the specialised word vectors for non-SimLex languages have high semantic content.}  
\label{tab:simlex-experiments-2}
\end{table}

\multicolumn{1}{c}{} & \multicolumn{4}{c}{\bf Machine Translations} \\
\multirow{2}{*}{\bf Word Vectors} & \multicolumn{2}{c|}{\bf Italian} & \multicolumn{2}{c}{\bf German} \\ 
 & Goals &  Requests & Goals &  Requests \\ \hline
\bf Monolingual Distributional Vectors  & 76.8  & 59.6 & 52.2 & 88.6 \\ 
\bf Monolingual Semantic Vectors        & 81.1 & 60.4 & 53.6 & \bf 90.4  \\ \hline
\bf Cross-Lingual Semantic Vectors      & 80.9 & \bf 75.5 & 54.7 & 88.0  \\ 
\bf + English Ontology Grounding        & \bf 81.5 & 69.4 & \bf 68.5 & 90.0 \\



\iffalse

10 percent:

{
    "prezzo": 0.599, 
    "joint": 0.38, 
    "request": 0.753, 
    "cibo": 0.486, 
    "area": 0.859
}

{
    "prezzo": 0.585, 
    "joint": 0.369, 
    "request": 0.743, 
    "cibo": 0.412, 
    "area": 0.882
}

{
    "prezzo": 0.547, 
    "joint": 0.305, 
    "request": 0.741, 
    "cibo": 0.381, 
    "area": 0.792
}

100 percent

{
    "prezzo": 0.897, 
    "joint": 0.753, 
    "request": 0.892, 
    "cibo": 0.809, 
    "area": 0.933
}

{
    "prezzo": 0.883, 
    "joint": 0.727, 
    "request": 0.896, 
    "cibo": 0.772, 
    "area": 0.933
}

{   
    "prezzo": 0.9,
    "joint": 0.712,
    "request": 0.876,
    "cibo": 0.769,
    "area": 0.944
}


\fi

%\subsection{Downstream Evaluation: Cross-Lingual Sentiment Analysis} 

%\textbf{NEW:} Using the multilingual Amazon reviews sentiment analysis dataset from \cite{Prettenhofer:10}, trying to get results competitive with those in \cite{Zhou:16}. If we can make a table similar to their Table 2 (for French and German, we omit Japanese), that would be ideal. 

%Most previous work trains bilingual document embeddings using the assorted collection of unlabelled Amazon reviews. We do not have that step. For now, if we can get decent results training on English, testing on German and French, that would be great. For that, we need a good model which uses our cross-lingual vectors, keeping them fixed during training to get models directly applicable to other languages present in the cross-lingual word vector collection. I can't find a model which keeps word embeddings fixed in the literature, so I implemented a CNN classifier which produces a document representation and uses it to classify the sentiment. I don't have competitive monolingual results yet, but there is evidence of transfer across languages. Also trying an LSTM, but training is much slower. 


\bf Bilingual EN-IT \cite{Mikolov:2013arxiv} & 0.32 & - & 0.26 & - \\
\bf Bilingual EN-IT \cite{Hermann:2014iclr} & 0.40 & - & 0.34 & - \\ 
\bf Bilingual EN-IT \cite{Gouws:2015icml} & 0.25 & - & 0.18  & - \\
\bf Bilingual EN-IT \cite{vulic:2016} & 0.32 & - & 0.27 & - \\
\bf Bilingual EN-IT \cite{Vulic:2016jair} & 0.23 & - & 0.25  & - \\ \hdashline
\bf Bilingual EN-DE \cite{Mikolov:2013arxiv} &  &  & - & - \\
\bf Bilingual EN-DE \cite{Hermann:2014iclr} &  &  & - & - \\ 
\bf Bilingual EN-DE \cite{Gouws:2015icml} &  &  & - & - \\
\bf Bilingual EN-DE \cite{vulic:2016} &  &  & - & - \\
\bf Bilingual EN-DE \cite{Vulic:2016jair} &  &  & - & - \\ \hline



English: 79.1, 90.6 
Italian: 69.3, 87.5
German:  50.7, 86.9 



iten 1 

{
    "food": 0.884, 
    "joint": 0.828, 
    "price range": 0.943, 
    "request": 0.92, 
    "area": 0.943
}


iten 2

{
    "food": 0.831, 
    "joint": 0.749, 
    "price range": 0.895, 
    "request": 0.908, 
    "area": 0.897
}


GloVe:

          goal.joint, acc, 2, a, 9689, 0.5123336
          requested.all, acc, 2, a, 5759, 0.9644035
          goal.food, acc, 2, a, 8919, 0.8341742
          goal.price range, acc, 2, a, 6708, 0.9320215
          goal.area, acc, 2, a, 8375, 0.6122985

Paragram:

          goal.joint, acc, 2, a, 9689, 0.7226752
          requested.all, acc, 2, a, 5759, 0.9645772
          goal.food, acc, 2, a, 8919, 0.8405651
          goal.price range, acc, 2, a, 6708, 0.9360465
          goal.area, acc, 2, a, 8375, 0.8995821




==> baselines_and_wiki.tex <==
\begin{table*}
\parbox{\columnwidth}{
\centering
\resizebox{1.0\columnwidth}{!}{%
\begin{tabular}{c|rc|rc}
\multirow{2}{*}{\bf Model} & \multicolumn{2}{c|}{\bf EN-IT} & \multicolumn{2}{c}{\bf EN-DE} \\ 
 & \bf EN & \bf  IT & \bf EN & \bf  DE \\ \hline
\bf \cite{Mikolov:2013arxiv} & 0.32 & 0.26 & 0.32 & 0.33 \\
\bf \cite{Hermann:2014iclr} & 0.40 & 0.34 & 0.38 & 0.35 \\ 
\bf \cite{Gouws:2015icml} & 0.25 & 0.18 & 0.25 & 0.14  \\
\bf \cite{vulic:2016} & 0.32 & 0.27 & 0.32 & 0.33 \\
\bf \cite{Vulic:2016jair} & 0.23 & 0.25 & 0.20 & 0.25 \\ \hline
\bf Bilingual \textsc{Attract-Repel} & \bf 0.70 & \bf 0.69 &  \bf 0.69 & \bf 0.61 \\ 
\end{tabular}}%
\caption{Comparison of the intrinsic quality (Multilingual SimLex-999) of the bilingual vector spaces produced by the \textsc{Attract-Repel} method with previously published work on constructing bilingual vector spaces. 
\label{tab:baselines}}
}
\hfill
\parbox{\columnwidth}{
\centering
\resizebox{1.0\columnwidth}{!}{%
\begin{tabular}{c|cccc}
\bf Word Vectors & \bf EN & \bf DE & \bf IT & \bf RU \\ \hline
\bf Distributional Vectors & 0.32 & 0.31 & 0.28 & 0.19 \\ %\hdashline
\bf \textsc{AR}: Monoling~Constraints & 0.61 & 0.48 & 0.53 & 0.52 \\
\bf \textsc{AR}: Monoling + Cross-Ling & \bf 0.66 & \bf 0.60 & \bf 0.65 & \bf 0.54 \\%
\end{tabular}}%
\caption{Multilingual SimLex-999. The effect of injecting linguistic constraints into distributional vectors trained on Wikipedia dumps instead of starting from well-known, high-quality collections of distributional word vectors.}
}
\end{table*}


==> bing-translation-baseline.tex <==
\begin{table*} %[!ht]
\centering
%\resizebox{1.0\linewidth}{!}{%
\def\arraystretch{0.95}
{\small
\begin{tabular}{c|rc|rc|rc}
\multirow{2}{*}{\bf Word Vectors} & \multicolumn{2}{c|}{\bf English} & \multicolumn{2}{c|}{\bf Italian} & \multicolumn{2}{c}{\bf German} \\ 
 & Goals &  Requests & Goals &  Requests & Goals &  Requests \\ \hline
\bf  Distributional Vectors & 78.6 & 90.4 & 56.3 & 85.9 &            59.1 & 83.7 \\
\bf  + Monolingual Constraints & 82.1 & 90.4 & 61.8 & 86.3 &         64.9  & 83.7 \\ 
\bf  ++ Cross-Lingual Constraints  & 79.9 & 90.6 &  63.1  &  85.3 &  64.8 & 83.9 \\ \hline

\bf Best Monolingual Scenario   & - & - & \bf 75.3 & 89.2 & \bf 55.7 & 86.1 \\ 
\end{tabular}%
}%}
\caption{NBT-CNN models' performance over the Italian and German WOZ 2.0 test sets Bing translated (back) to English. The first three models were trained on the English WOZ 2.0 training data. The final line shows the best performance achieved by the NBT models trained and evaluated in Italian and German. % The first baseline model uses no semantic dictionary.
\label{tab:bing_baseline}} 
\end{table*}

==> constraints-full.tex <==
\begin{table*}
\def\arraystretch{1.0}
\centering
%\resizebox{2.05\columnwidth}{!}{%
{\small
\begin{tabular}{c|cccc|cccc|cccc}
& \bf EN & \bf DE & \bf NL & \bf SV & \bf FR & \bf ES & \bf IT & \bf PT & \bf RU & \bf PL & \bf SH & \bf BG \\ \hline

\bf EN  & 64/1 & 25/~1 & 31/2 & 21/1 & ~36/2 & ~32/2 & 36/2 & 26/1 & 120/1 & 28/1 & 19/1 & 14/1\\
\bf DE  & 25/1 & 14/0 & 29/1 & 22/1 & ~29/1 & ~27/1 & 28/1 & 22/1 & 18/1 & 23/1 & 17/1 & 13/0\\
\bf NL  & 31/2 & 29/1 & 68/3 & 24/1 & ~35/2 & ~32/2 & 34/2 & 26/1 & 20/1 & 28/1 & 20/1 & 15/1\\
\bf SV  & 21/1 & 22/1 & 24/1 & ~0/0 & ~24/1 & ~22/1 & 23/1 & 19/1 & 14/1 & 20/1 & 15/1 & 11/0\\ \hline
\bf FR  & 36/2 & 28/1 & 35/2 & 24/1 & 103/1 & ~36/2 & 39/2 & 28/1 & 22/1 & 31/1 & 21/1 & 15/1\\
\bf ES  & 32/2 & 27/1 & 32/2 & 22/1 & ~36/2 & 114/0 & 34/2 & 26/1 & 20/1 & 28/1 & 19/1 & 14/1\\
\bf IT  & 35/2 & 28/1 & 34/2 & 23/1 & ~39/2 & ~34/2 & 16/1 & 28/2 & 22/1 & 30/2 & 21/1 & 15/1\\
\bf PT  & 26/1 & 22/1 & 26/1 & 19/1 & ~28/1 & ~26/1 & 28/2 & 72/0 & 16/1 & 23/1 & 17/1 & 12/1\\ \hline
\bf RU  & 20/1 & 18/1 & 20/1 & 14/1 & ~22/1 & ~20/1 & 22/1 & 16/1 & ~5/0 & 17/1 & 12/1 & ~9/0\\
\bf PL  & 28/1 & 23/1 & 28/1 & 20/1 & ~31/1 & ~28/1 & 30/2 & 23/1 & 17/1 & 39/0 & 19/1 & 13/1\\
\bf SH  & 19/1 & 17/1 & 20/1 & 15/1 & ~21/1 & ~19/1 & 21/1 & 16/1 & 12/1 & 19/1 & ~0/0 & 10/1\\
\bf BG  & 14/1 & 13/0 & 15/1 & 11/0 & ~15/1 & ~14/1 & 15/1 & 12/1 & ~9/0 & 13/1 & 10/1 & 18/0\\
 \end{tabular}}%
%}
\caption{Linguistic constraint counts (in tens of thousands). For each language pair, the two figures show the number of synonymy and antonymy constraints. Monolingual similarity constraints were extracted from PPDB, whereas cross-lingual similarity and both monolingual and cross-lingual antonymy were extracted from BabelNet. }

\label{tab:constraint-count}
\end{table*}


==> dst-performance-en.tex <==
\begin{table*} [!ht]
\centering
\resizebox{2.05 \columnwidth}{!}{%
\def\arraystretch{0.95}
{\small
\begin{tabular}{l|rc|rc|rc}
\multicolumn{1}{c|}{\multirow{2}{*}{\bf Word Vectors}} & \multicolumn{2}{c|}{\bf English} & \multicolumn{2}{c|}{\bf Italian} & \multicolumn{2}{c}{\bf German} \\ 
 & Goals &  Requests & Goals &  Requests & Goals &  Requests \\ \hline
\bf  EN-IT/EN-DE \cite{Mikolov:2013arxiv} & 78.2 & & 71.1 & 85.3 & 50.5 & 83.5 \\
\bf  EN-IT/EN-DE \cite{Hermann:2014iclr} & 71.7 & & 69.3 & 86.5 & 44.7 & 84.1 \\ 
\bf  EN-IT/EN-DE \cite{Gouws:2015icml} & 75.0 &  & 68.4 & 88.0 & 45.4  & 82.4  \\
\bf  EN-IT/EN-DE \cite{vulic:2016} & &  & 71.8 & 87.8 & 50.5 & 83.5  \\
\bf  EN-IT/EN-DE \cite{Vulic:2016jair} & & & 69.0 & \bf 89.6 & 38.2 & 82.5 \\ \hline %\hline

\bf Monolingual Distributional Vectors & 77.6 & 90.4  &  71.2    & 87.6 & 46.6 & 85.1  \\ 
\bf  \textsc{Attract-Repel}: Monolingual Constraints & 80.9 &  90.4 &  72.7    &  \bf 89.6 & 52.4 &  87.1  \\ 
\bf  \textsc{Attract-Repel}: + Cross-Lingual Constraints &  80.3 & 90.6  &  75.3 & 89.2 & 55.7 & 86.1 \\ \hline
\bf \textsc{Attract-Repel}: English Ontology Grounding & \bf  82.8 & \bf 90.8 & \bf 77.1 & 89.4 & \bf 57.7 & \bf 88.0 \\
\end{tabular}
}}
\caption{NBT-CNN model's WOZ 2.0 accuracies for: \textbf{a)} joint goals; and \textbf{b)} turn-level requests. Each line shows the performance of NBT models trained using the Italian or German parts of the respective cross-lingual vector space. The cross-lingual specialisation for the last two experiments was performed using the four SimLex languages.   % The first baseline model uses no semantic dictionary.
\label{tab:dst_performance}} 
\end{table*}




==> dst-performance.tex <==
\begin{table*} 
\centering
%\resizebox{2.05 \columnwidth}{!}{%
\def\arraystretch{0.93}
{\small
\begin{tabular}{l|c|c|c}
\multicolumn{1}{c|}{\multirow{1}{*}{\bf Word Vector Space}} &  \bf English &  {\bf ~Italian~} & {\bf ~German~ } \\  \hline
\bf  EN-IT/EN-DE \cite{Mikolov:2013arxiv} & 78.2 & 71.1 & 50.5  \\
\bf  EN-IT/EN-DE \cite{Hermann:2014iclr} & 71.7  & 69.3 & 44.7 \\ 
\bf  EN-IT/EN-DE \cite{Gouws:2015icml}  & 75.0 & 68.4 &  45.4    \\
\bf  EN-IT/EN-DE \cite{vulic:2016}  &  81.6 &  71.8 &  50.5  \\
\bf  EN-IT/EN-DE \cite{Vulic:2016jair} &  72.3 & 69.0  & 38.2 \\ \hline %\hline
\bf Monolingual Distributional Vectors & 77.6 &  71.2    & 46.6   \\ 
\bf  \textsc{Attract-Repel}: Monolingual Specialisation & 80.9 &  72.7    &  52.4  \\  
\bf  \textsc{Attract-Repel}: EN-DE-IT-RU Vector Space & 80.3 &  75.3 &  55.7 \\ 
\bf  + English Ontology Grounding & \bf 82.8 & \bf 77.1 &  \bf 57.7  \\
\end{tabular}
}%}
\caption{NBT-CNN model's joint goal accuracies across the three languages in Multilingual WOZ 2.0. Each figure shows the performance of the NBT model trained using the subspace of the given vector space corresponding to the target language. For the English baseline figures, we show the stronger of the EN-IT / EN-DE figures. %The experiments shown in the last two rows make use of the four-lingual EN-DE-IT-RU vector space.   % The first baseline model uses no semantic dictionary.
\label{tab:dst_performance} \vspace{-4mm}} 
\end{table*}


\iffalse

78.2, 77.7
68.7, 71.7
71.5, 75.0
81.6 , 79.8
69.5, 72.3

\fi



==> dst-with-requests.tex <==
\begin{table*} [!ht]
\centering
%\resizebox{2.05 \columnwidth}{!}{%
\def\arraystretch{0.95}
{\small
\begin{tabular}{l|rc|rc}
\multicolumn{1}{c|}{\multirow{2}{*}{\bf Word Vectors}} & \multicolumn{2}{c|}{\bf Italian} & \multicolumn{2}{c}{\bf German} \\ 
 & Goals &  Requests & Goals &  Requests  \\ \hline
\bf  EN-IT/EN-DE \cite{Mikolov:2013arxiv} & 71.1 & 85.3 & 50.5 & 83.5 \\
\bf  EN-IT/EN-DE \cite{Hermann:2014iclr} & 69.3 & 86.5 & 44.7 & 84.1 \\ 
\bf  EN-IT/EN-DE \cite{Gouws:2015icml}  & 68.4 & 88.0 & 45.4  & 82.4  \\
\bf  EN-IT/EN-DE \cite{vulic:2016}  & 71.8 & 87.8 & 50.5 & 83.5  \\
\bf  EN-IT/EN-DE \cite{Vulic:2016jair} & 69.0 & \bf 89.6 & 38.2 & 82.5 \\ \hline %\hline

\bf Monolingual Distributional Vectors &  71.2    & 87.6 & 46.6 & 85.1  \\ 
\bf  \textsc{Attract-Repel}: Monolingual Constraints &  72.7    &  \bf 89.6 & 52.4 &  87.1  \\ 
\bf  \textsc{Attract-Repel}: + Cross-Lingual Constraints &  75.3 & 89.2 & 55.7 & 86.1 \\ \hline
\bf \textsc{Attract-Repel}: English Ontology Grounding & \bf 77.1 & 89.4 & \bf 57.7 & \bf 88.0 \\
\end{tabular}
}%}
\caption{NBT-CNN model's WOZ 2.0 accuracies for: \textbf{a)} joint goals; and \textbf{b)} turn-level requests. Each line shows the performance of NBT models trained using the Italian or German parts of the respective cross-lingual vector space. The cross-lingual specialisation for the last two experiments was performed using the four SimLex languages.   % The first baseline model uses no semantic dictionary.
\label{tab:dst_performance}} 
\end{table*}





==> four-lang-transpose.tex <==

\begin{table} 
\def\arraystretch{0.93}
\centering
%\resizebox{1.0\columnwidth}{!}{%
{\small
\begin{tabular}{c|cccc}
%& \multicolumn{4}{c|}{ SimLex Languages} &  \multicolumn{8}{c}{ Non-SimLex Languages} \\
     & \bf  English  & \bf  German   & \bf  Italian  & \bf  Russian \\ \hline
\bf EN   & 0.65 & \bf 0.61 & \bf 0.69 & \bf 0.63 \\
\bf DE   & \bf 0.69 & 0.43 & \bf 0.65 & \bf 0.59 \\ 
\bf IT   & \bf 0.70 & \bf 0.58 & 0.56 & \bf 0.62 \\
\bf RU   & \bf 0.70 & \bf 0.56 & \bf 0.64 &  0.56 \\ \hdashline
\bf NL   & \bf 0.70 & \bf 0.55 & \bf 0.67 & \bf 0.61 \\
\bf FR   & \bf 0.72 & \bf 0.60 & \bf 0.68 & \bf 0.61 \\
\bf ES   & \bf 0.72 & \bf 0.59 & \bf 0.68 & \bf 0.62 \\
\bf PT   & \bf 0.70 & \bf 0.56 & \bf 0.66 & \bf 0.58 \\ 
\bf PL   & \bf 0.70 & \bf 0.54 & \bf 0.66 & \bf 0.60 \\
\bf BG   & \bf 0.68 & \bf 0.52 & \bf 0.62 & \bf 0.61 \\ \hdashline

\bf SH   & \bf 0.69 & \bf 0.53 & \bf 0.63 & \bf 0.59 \\
\bf SV   & \bf 0.70 & \bf 0.55 & \bf 0.63 & \bf 0.60 \\
\bf HE   & & & & \\
\bf GA & & & & 
% Tying to English:

% EN-DE: 0.69, 0.58
% EN-IT: 0.70, 0.69
% EN-RU: 0.69, 56

% Tied to German:

% DE-EN: 0.61, 0.60 (EN-DE, always in order en-de-it-ru if only two) 
% DE-IT: 0.59. 0.66
% DE-RU: 0.56, 0.52

% Tying to Italian:

% EN-IT: 0.66, 0.67
% DE-IT: 0.55, 0.66
% IT-RU: 0.63, 0.55

% Tying to Russian - running now: 

% IT-RU: 0.63, 0.63 
% DE-RU: 0.49, 0.60
% IT-RU: 0.63, 0.63

% EN-HE-GA: 

% English reaches 0.67 

\end{tabular}%}%
}
\caption{Bilingual semantic specialisation for the four SimLex languages combined with each of the twelve languages. The four figures on the first diagonal indicate monolingual specialisation for the SimLex languages. Figures in bold indicate improvements over these baselines. \vspace{-4mm} }

\label{tab:four-lang-expansion}
\end{table}

==> german-grounding.tex <==
36  28.0
60	31.1
120	38.4
180	42.6
240	44.2
300 48.4
360 52.8
420 55.0
480 56.2
540 56.5
600 58.0

==> italian-grounding.tex <==
36 57.6
60  59.8
120	64.7
180	65.4
240	69.9
300	71.9
360	74.7
420	76.7
480 77.0
540 78.5
600 78.7

==> machine-reading.tex <==


\paragraph{Machine Reading / Question Answering}


\begin{table} [!ht]
\centering
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{c|cc}
 
\bf Model & \bf Exact Match & \bf F-score \\ \hline

\bf Match-LSTM-boundary (GloVe) & 60.5 &	70.7 \\
\bf Match-LSTM-boundary (cross-lingual) & 63.3D & 73.1D \\ \hline
\bf Match-bi-LSTM-ensemble (GloVe) & 67.9 & 77.0 \\ 
\bf High Score \cite{Xiong:16} & 71.6 & 80.4 \\

\end{tabular}%
}
\caption{Stanford QA performance comparison. We compare the Match-LSTM model powered by GloVe vectors to the same model making use of our best English vectors. The final line shows the best validation score achieved so far. \textbf{Table shows current validation (marked with D).} }

\label{tab:machine-reading}
\end{table}

\cite{Wang:16} propose a method for the Stanford QA \cite{Rajpurkar:16} dataset which keeps word vectors fixed. We analyse what happens once their default GloVe vectors are replaced by our semantically specialised ones.  Their best interpolated score on the test set is: 67.9 on exact matches and 77.0 for f-score. This is a bi-LSTM ensemble of five with a complicated interpolation scheme. Their best scores with the singer boundary model that we are training is 60.5, 70.7, which is lower than our validation: we've got 63.3, 73.0 as the best score on the development set after 18 (out of 30) epochs. 5 epochs left, so half a day left (done by Friday evening). If there's no over-fitting we are in good shape. Comparison to high-score in Table \ref{tab:machine-reading}; we should do this properly (bidirectional LSTM + ensemble method), and then try to see if we get more competitive results for Stanford-QA. 

